Wireless millimeterwave electro-optics on thin film lithium niobate

The rapid growth of global data traffic is accelerating the need for ultra-broadband communication technologies, particularly in cloud infrastructure and emerging 6G wireless systems. Optical computing and quantum information processing also demand fast, scalable ways to interface optical and electronic signals. Integrated electro-optic modulators provide a compact and efficient solution, but extending their operation into the millimeterwave (mmWave) range with wide bandwidth and compatibility with wireless signals remains a significant challenge. Bulky electrical packaging and high mmWave losses remain primary barriers to scalability. Here, we demonstrate a wireless and wideband electro-optic modulation architecture that directly interfaces mmWaves with optical signals, eliminating the need for impedance-matched mmWave probes and cables. By integrating an on-chip antenna with a co-designed transmission line on thin-film lithium niobate platform, we achieve wideband modulation across the WR9.0 (82-125 GHz) and WR2.8 (240-380 GHz) bands. The wideband nature of our modulator enables the device to function as a high-speed detector of mmWave carriers modulated up to 6~GHz and achieves a flat and wide response, a key requirement for 6G and high-speed mmWave sensing. By configuring the antenna-coupled transmission line to operate as a cavity, our wireless platform enables triply resonant electro-optic frequency comb generation with mode spacing of 123.2 GHz and 307.9 GHz. Extracted single-photon electro-optic coupling rates of $g_{0} =2\pi\times 4.98$ kHz and $2\pi\times 9.93$ kHz, at 123.2 and 307.9 GHz, respectively, demonstrate favorable scaling with mmWave frequency. These results introduce a new class of wireless electro-optic devices for high-speed modulation, detection, and frequency comb generation, with impactful applications in communications, sensing, and quantum technologies.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
